Deterministic Conjunction Tracking in Long-term Space Debris Simulations

Numerical simulations are at the center of predicting the space debris environment of the upcoming decades. In light of debris generating events, such as continued anti-satellite weapon tests and planned mega-constellations, accurate predictions of the space debris environment are critical to ensure the long-term sustainability of critical satellite orbits. Given the computational complexity of accurate long-term trajectory propagation for a large number of particles, numerical models usually rely on Monte-Carlo approaches for stochastic conjunction assessment. On the other hand, deterministic methods bear the promise of higher accuracy and can serve to validate stochastic approaches. However, they pose a substantial challenge to computational feasibility. In this work, we present the architecture and proof of concept results for a numerical simulation capable of modeling the long term debris evolution over decades with a deterministic conjunction tracking model. For the simulation, we developed an efficient propagator in modern C++ accounting for Earth's gravitational anomalies, solar radiation pressure, and atmospheric drag. We utilized AutoPAS, a sophisticated particle container, which automatically selects the most efficient data structures and algorithms. We present results from a simulation of 16 024 particles in low-Earth orbit over 20 years. Overall, conjunctions are tracked for predicted collisions and close encounters to allow a detailed study of both. We analyze the runtime and computational cost of the simulation in detail. In summary, the obtained results show that modern computational tools finally enable deterministic conjunction tracking and can serve to validate prior results and build higher-fidelity numerical simulations of the long-term debris environment.

==> s-conc.tex <==

\section{Conclusion} Figure~\ref{fig:fig1} Nunc ut arcu sit amet lectus facilisis aliquet non
a eros. Sed commodo pulvinar sem vel faucibus. Proin nisl justo, placerat vel ante sed, rutrum
venenatis felis. Phasellus nulla nisl, aliquet ut mi at, accumsan sollicitudin enim. Morbi ut
sodales mauris, in fringilla odio. Duis eros arcu, pretium eget vehicula a, viverra non nunc.
Ut feugiat ultrices blandit. Quisque efficitur quis nunc eu commodo. Aenean quis ipsum at risus
mollis placerat. Vestibulum ut feugiat lacus, in semper tellus. Sed consequat libero quis orci
porta fermentum. Donec placerat vehicula sapien ullamcorper ullamcorper. Sed blandit tempus
turpis ut vulputate. Pellentesque sit amet ullamcorper sem, sit amet sollicitudin arcu. 

Figure \ref{fig:fig2} suspendisse porta pulvinar ante, vitae tincidunt justo pharetra non. Sed
blandit id felis at efficitur. Sed vehicula, nunc quis efficitur convallis, sapien leo iaculis
sapien, vitae molestie diam leo a turpis. In dictum eget sapien nec pharetra. Praesent diam
risus, scelerisque ut fermentum ut, sagittis id tortor. Donec suscipit a erat quis lobortis.
Vivamus mollis tempor neque ut tincidunt. In dictum, dui id tempor efficitur, metus arcu
vulputate leo, congue efficitur arcu enim eget tellus. In mauris nulla, auctor ut posuere non,
feugiat ac ex. Duis quis orci non neque ullamcorper sodales sed sed nisl. Proin fermentum
finibus neque, non interdum magna commodo dignissim. Phasellus consequat ex molestie vehicula
tincidunt. Phasellus fermentum bibendum ultrices. 

Proin convallis ante quis tellus hendrerit tempus. Sed eleifend justo id
neque condimentum, ut bibendum ipsum dapibus. Proin ut mollis velit. Aenean porttitor eu enim
vitae viverra. Fusce eros leo, accumsan quis dapibus non, porttitor sit amet mauris. 

\endinput



==> s-sec1.tex <==

\section{Section Title} Nullam quis convallis dolor. Nullam magna sapien, tincidunt nec eros nec,
semper pharetra nunc. In pellentesque pretium tincidunt. Vestibulum in nulla arcu. Donec vel nulla
eleifend metus pharetra elementum ac ac ligula. Vivamus rhoncus, nibh id maximus bibendum, enim
lacus egestas erat, quis fermentum ex orci ac massa. Phasellus vestibulum imperdiet mi, vitae
malesuada massa sodales quis. Pellentesque molestie arcu ut tortor vestibulum, a gravida diam
efficitur. Nulla ut lorem ac eros tincidunt elementum. Curabitur vestibulum auctor vestibulum.
Nullam molestie mauris nec justo accumsan, vitae accumsan sem varius. Quisque sagittis neque sed
enim efficitur, eu consectetur odio volutpat. Pellentesque arcu mauris, maximus venenatis gravida
nec, bibendum ut mauris. Cum sociis natoque penatibus et magnis dis parturient montes, nascetur
ridiculus mus~\cite{SampleRef3}.  

\endinput



==> s-sec2.tex <==

\section{Section Title} Etiam porttitor aliquam erat, commodo interdum leo placerat at. Cras non
feugiat felis. Duis nunc nisi, consequat at lorem nec, accumsan porta sapien. Proin cursus est
quis eleifend feugiat. Vestibulum urna lectus, accumsan quis sapien sit amet, dignissim porttitor
velit. Sed ut porta ipsum. Morbi viverra massa eu tellus vehicula, ac sodales risus ultricies.
Mauris mattis id dolor in posuere.

Sed non odio sagittis, tincidunt tellus vitae, lobortis turpis. Cras pellentesque hendrerit
risus at commodo. Nulla in scelerisque justo. Ut tincidunt tristique tortor, quis porta tortor
ultricies vitae. Proin non nibh sit amet nunc suscipit blandit. Maecenas in molestie nisi.
Maecenas dictum quam ut dictum consequat. Etiam sit amet malesuada nibh. Proin ornare malesuada
elit. Morbi pretium, arcu eu sodales pellentesque, leo dui elementum ex, vulputate ullamcorper
metus orci et dui. Sed quis pharetra nisl, sit amet convallis neque. Phasellus eget lectus dolor.  

\begin{figure*}[t!]
    \begin{center}
        \includegraphics[width=0.95\textwidth, height=3.65in]{placeholder_fig}
        \caption{\small{Caption goes here.}}
        \label{fig:fig1}
    \end{center}
\end{figure*}
%NOTE: for figures to span across the two columns use \begin{figure*} ... \end{figure*} or without * for single column

\endinput



==> s-sec3.tex <==

\section{Section Title}  Duis at tincidunt orci. In dictum viverra sapien, ut lacinia odio rutrum at.
Nam ut ipsum congue, condimentum massa eu, dictum tellus. Nulla eu sem ac turpis tincidunt varius
sollicitudin ut massa. Duis consectetur eu est id vestibulum. Donec et nibh elementum, efficitur
dolor a, accumsan mauris. Quisque et enim faucibus, cursus magna gravida, rutrum velit. Proin sed
aliquam mi. Suspendisse potenti. Donec faucibus, libero aliquet lacinia viverra, dui turpis ornare
turpis, viverra pellentesque metus nulla sit amet ipsum. Quisque nec magna eu sapien cursus commodo.
Morbi pellentesque quam eget quam volutpat, in tempus felis imperdiet. Quisque non tortor arcu.

\begin{figure}[h!]
    \begin{center}
        \includegraphics[width=0.47\textwidth]{placeholder_fig}
        \caption{\small{Caption goes here.}}
        \label{fig:fig2}
    \end{center}
\end{figure}

Maecenas commodo varius odio id gravida. Fusce nec dapibus mauris, nec sollicitudin nisi. Ut nec
suscipit enim. Cras tincidunt lacus placerat placerat eleifend. Cras elit sapien, hendrerit nec
augue non, pulvinar interdum est. Ut viverra posuere lectus, quis mattis mi condimentum sed. Nunc
in nisl id risus tincidunt interdum tempus ac arcu. Nulla sollicitudin convallis interdum. Quisque
vitae congue mauris.

\endinput


